Constructing Depth-Optimum Circuits for Adders and AND-OR Paths

We examine the fundamental problem of constructing depth-optimum circuits for binary addition. More precisely, as in literature, we consider the following problem: Given auxiliary inputs $t_0, \dotsc, t_{m-1}$, so-called generate and propagate signals, construct a depth-optimum circuit over the basis {AND2, OR2} computing all $n$ carry bits of an $n$-bit adder, where $m=2n-1$. In fact, carry bits are AND-OR paths, i.e., Boolean functions of the form $t_0 \lor ( t_1 \land (t_2 \lor ( \dots t_{m-1}) \dots ))$. Classical approaches construct so-called prefix circuits which do not achieve a competitive depth. For instance, the popular construction by Kogge and Stone is only a $2$-approximation. A lower bound on the depth of any prefix circuit is $1.44 \log_2 m$ + const, while recent non-prefix circuits have a depth of $\log_2 m$ + $\log_2 \log_2 m$ + const. However, it is unknown whether any of these polynomial-time approaches achieves the optimum depth for all $m$. We present a new exponential-time algorithm solving the problem optimally. The previously best exact algorithm with a running time of $\mathcal O(2.45^m)$ is viable only for $m \leq 29$. Our algorithm is significantly faster: We achieve a running time of $\mathcal O(2.02^m)$ and apply sophisticated pruning strategies to improve practical running times dramatically. This allows us to compute optimum circuits for all $m \leq 64$. Combining these computational results with new theoretical insights, we derive the optimum depths of $2^k$-bit adder circuits for all $k \leq 13$, previously known only for $k \leq 4$. In fact, we solve a more general problem occurring in VLSI design: $delay$ optimization of a $generalization$ of AND-OR paths where AND and OR do not necessarily alternate. Our algorithm arises from our new structure theorem which characterizes delay-optimum generalized AND-OR path circuits.

==> fractional_ats.tex <==
\section{From Integral to Fractional Arrival Times} \label{gen-sec-frac-ats}

In \cref{n-times-int-general}, we present
a generic approach to extend a given circuit construction algorithm
which works on integral arrival times only to fractional arrival times
while only losing a running time factor of $\mathcal O(n)$.
In \cref{thm-binary-search-general},
we improve the additional running time factor to $\mathcal O(\log_2 n)$
using a specific binary search.

\begin{definition}
Consider a Boolean function $f \colon \I^n \to \I$
with input variables $x_0, \dotsc, x_{n-1}$
and let $S$ denote a non-empty set of circuits realizing $f$.
We call a circuit $C \in S$ an \define{$S$-optimum circuit} for $f$
with respect to arrival times
$a(x_0), \dotsc, a(x_{n-1}) \in \R$
if $\delay(C; a) \leq \delay(C'; a)$ for all $C' \in S$.
We say that an algorithm $A$ is \define{$S$-optimum}
if it always computes an $S$-optimum circuit for $f$.
\end{definition}

For example,
let $f$ be a generalized \aop{} $f = h(t; \Gamma)$ with inputs $t = \Bkt{t_0, \dotsc, t_{m-1}}$
and gate types $\Gamma = \Bkt{\circ_0, \dotsc, \circ_{m-2}}$
and $S$ be the set of all formula circuits for $f$.
Then, in \cref{alg::opt_dp},
we will see an $S$-optimum algorithm.
However, in our practical implementation of \cref{alg::opt_dp} which applies
the speedup techniques from \cref{sec::opt-impl},
we will assume that the arrival times are integral.
Hence, in this \lcnamecref{gen-sec-frac-ats},
we will show how to extend an $S$-optimum algorithm $A$
which is defined only for integral arrival times
to fractional arrival times.
For this, we need the following \lcnamecref{S-opt-lemma}.

\begin{lemma} \label{S-opt-lemma}
 Given a Boolean function $f$ with input variables $x_0, \dotsc, x_{n-1}$,
 a non-empty set $S$ of circuits for $f$,
 the following statements are fulfilled:
 \begin{enumerate}
  \item Consider arrival times $a$ and a number $\alpha \in \R$.
   Let arrival times $\tilde a$ be given by
   $\tilde a(x_i) = a(x_i) + \alpha$ for each $i \in \set{0, \dotsc, n-1}$.
   Then, a circuit $C \in S$ is $S$-optimum for arrival times $a$
   with delay $d \in \R$
   if and only if it is
   $S$-optimum for arrival times $\tilde a$ with delay $d + \alpha \in \R$. \label{cond-shift}
  \item Consider arrival times $a, \tilde a$ with $a(x_i) \leq \tilde a(x_i)$
   for all $i \in \set{0, \dotsc, n-1}$
   and two circuits $C, \widetilde C \in S$.
   Assume that $C$ is $S$-optimum with respect to arrival times $a$.
   Then, we have $\delay(C; a) \leq \delay(\widetilde C; \tilde a)$. \label{cond-mon}
 \end{enumerate}
\begin{proof}
 The first statement holds as for any circuit $C$, we have
 $\delay(C; \tilde a) = \delay(C; a) + \alpha$.

 To see the second statement, note that $\widetilde C$ is a circuit for $f$
 with delay $\delay(\widetilde C; a) \leq \delay(\widetilde C; \tilde a)$
 as $a(x_i) \leq \tilde a(x_i)$ for each $i \in \set{0, \dotsc, n-1}$.
 As $C$ is $S$-optimum for arrival times $a$ and $\widetilde{C} \in S$,
 we have $\delay(C; a) \leq \delay(\widetilde C; a)$.
 Together, this yields the second statement.
\end{proof}
\end{lemma}

\begin{proposition} \label{n-times-int-general}
 Consider a Boolean function $f \colon \I^n \to \I$
 with input variables $x_0, \dotsc, x_{n-1}$
 and a non-empty set $S$ of circuits for $f$.
 Assume that algorithm $A$ is an $S$-optimum algorithm
 with running time $\mathcal O(r(n))$
 which is only defined for integral input arrival times.
 Then, there is an $S$-optimum algorithm $A'$ for arbitrary fractional input arrival times
 with running time $\mathcal O(r(n) n)$.
 We call $A'$ the \define{linear-search extension}
 of algorithm $A$.
 \begin{proof}
 By \cref{S-opt-lemma}, \labelcref{cond-shift},
 we may assume that all arrival times are non-negative.

 Given a fractional number $b \in \R$, let $\fp(b) := b - \BktD{b} \in [0, 1)$
 denote the fractional part of $b$.
 Let
 $F := \BktC{\fp(a(x_i)) \where{} i \in \{0, \dotsc, n-1\}}$.

 Consider the following algorithm $A'$:
 For each $\alpha \in F$, we create an instance with integral arrival times
 \begin{equation} \label{def-a-alpha}
 a_\alpha(x_i) = \begin{cases}
               \BktU{a(x_i)} & \text{ if } \fp(a(x_i)) > \alpha \\
               \BktD{a(x_i)} & \text{ otherwise}
              \end{cases}
   \quad \text{ for each } i \in \{0, \dotsc, m-1\}\,.
\end{equation}
 For every $\alpha \in F$, we apply algorithm $A$
 to the instance with modified arrival times $a_\alpha(x_i) \in \N$
 to obtain a circuit $C_\alpha \in S$ realizing $f$.
 We output a circuit $C_{\alpha^*}$ which has best delay with respect to arrival times $a$
 among all circuits created.

 As $|F| \leq n$ and the running time of algorithm $A$ is $r(n)$ by assumption,
 the running time algorithm $A'$ is at most $\mathcal O(r(n)n)$.

 In order to prove $S$-optimality of $A'$,
 for each $\alpha \in F$,
 also consider the instance with arrival times
 $\tilde{ a}_{\alpha}(x_i)$ resulting from $a(x_i)$
 by rounding up to the next fractional number $b_i$ with $\fp(b_i) = \alpha$.
 Note that for each $i \in \set{0, \dotsc, n-1}$, we have
 {
 \newcommand{\aw}{4}
 \begin{align} \label{a = tilde a - alpha}
   a_\alpha(x_i) \ca{\aw}{=} \tilde a_{\alpha}(x_i) - \alpha\,.
 \shortintertext{This implies}
 \label{bound-delay-alpha-a}
  \delay(C_{\alpha}; a)
  \ca{\aw}{\overset{a \leq \tilde a_{\alpha}}{\leq}}
    \delay(C_{\alpha}; \tilde{a}_{\alpha})
  \overset{\labelcref{a = tilde a - alpha}}{=} \delay(C_{\alpha}; a_{\alpha}) + \alpha\,.
 \end{align}
 }

 Now, consider a circuit $C \in S$
 with optimum delay $d := d(C; a) \in \R$ among all circuits in $S$.
 Consider an input $x_j$ for which there is a path
 $P \colon x_j \rightsquigarrow \cktout(C)$ with
 $a(x_j) + |P| = d$.
 In particular, we have $\fp(x_j) = \fp(d)$.
 Let $\alpha^* := \fp(x_j)$.
 We will show that $C_{\alpha^*}$ fulfills $\delay(C_{\alpha^*}; a) = d$.

 Note that $\delay(C; \tilde a_{\alpha^*}) = d$.
 Furthermore, we have
 \begin{equation} \label{delay-C-a-alpha*}
 \delay(C; a_{\alpha^*}) \overset{\labelcref{a = tilde a - alpha}}{=}
   \delay(C; \tilde a_{\alpha^*}) - \alpha^* = d - \alpha^*\,.
 \end{equation}

 As the circuit $C$ is $S$-optimum for arrival times $a$,
 and, by $S$-optimality of algorithm $A$,
 the circuit $C_{\alpha^*}$ is $S$-optimum for arrival times $a_{\alpha^*}$,
 we obtain
 \begin{equation}
  d \leq \delay(C_{\alpha^*}; a)
     \overset{\labelcref{bound-delay-alpha-a}}{\leq} \delay(C_{\alpha^*}; a_{\alpha^*}) + \alpha^*
     \leq \delay(C; a_{\alpha^*}) + \alpha^*
     \overset{\labelcref{delay-C-a-alpha*}}{=} d\,. \label{delay-alpha-eq}
  \end{equation}
 So in fact, all inequalities in \cref{delay-alpha-eq} are fulfilled with equality
 and $C_{\alpha^*}$ is $S$-optimum with respect to arrival times $a$.
 Hence, our algorithm $A'$ is $S$-optimum.
 \end{proof}
\end{proposition}

For improving the running time of algorithm $A'$,
we need the essential property that algorithm $A$ is monotone
in the following sense:

\begin{observation}\label{obs-alpha-monotone}
 Consider again the proof of \cref{n-times-int-general},
 in particular the set $F := \BktC{\fp(a(x_i)) \where{} i \in \{0, \dotsc, m\}}$
 and the modified arrival times $a_{\alpha}$ defined in \cref{def-a-alpha}
 for each $\alpha \in F$.
 Then, for $\alpha_1, \alpha_2 \in F$ with $\alpha_1 < \alpha_2$,
 we have $a_{\alpha_1}(x_i) \geq a_{\alpha_2}(x_i) \geq a_{\alpha_1}(x_i) - 1$ for each $i \in \set{0, \dotsc, m-1}$.
 As in the proof, let $C_{\alpha_1}, C_{\alpha_2} \in S$
 be the $S$-optimum circuits for arrival times $a_{\alpha_1}$ and $a_{\alpha_2}$
 computed by algorithm $A$, respectively.
 By \cref{S-opt-lemma}, \labelcref{cond-shift},
 the circuit $C_{\alpha_1}$ is $S$-optimum for arrival times $a_{\alpha_1}(x_i) - 1$.
 Note that
 $\delay(C_{\alpha_1}; a_{\alpha_1} - 1) = \delay(C_{\alpha_1}; a_{\alpha_1}) - 1$.
 By \cref{S-opt-lemma}, \labelcref{cond-mon},
 we thus have
 \[\delay(C_{\alpha_1}; a_{\alpha_1})
   \geq \delay(C_{\alpha_2}; a_{\alpha_2})
   \geq \delay(C_{\alpha_1}; a_{\alpha_1}) - 1\,.\]
\end{observation}

Using this \lcnamecref{obs-alpha-monotone},
we can derive our final algorithm for
instances with fractional arrival times.

\begin{table}
 \centering
 \begin{tabular}{lllllll}
  $\alpha$                                & 0.0 & 0.3 & 0.4 & 0.5 & 0.7 & 0.8 \\ \midrule
  $\delay(C_\alpha; a_{\alpha})$          & 6   & 6   & 6   & 5   & 5   & 5 \\
  $\delay(C_\alpha; a_{\alpha}) + \alpha$ & 6.0 & 6.3 & 6.4 & 5.5 & 5.7 & 5.8 \\ \bottomrule
 \end{tabular}
 \caption[Example for the binary-search extension of an algorithm.]{
    Example illustrating the proof of \cref{thm-binary-search-general}.
    We have $\alpha^* = 0.5$.}
 \label{table-binary}
\end{table}

\begin{theorem} \label{thm-binary-search-general}
 Consider a Boolean function $f \colon \I^n \to \I$
 with input variables $x_0, \dotsc, x_{n-1}$
 and a non-empty set $S$ of circuits for $f$.
 Assume that algorithm $A$ is an $S$-optimum algorithm
 with running time $\mathcal O(r(n))$
 which is only defined for integral input arrival times.
 Then, there is an $S$-optimum algorithm $A'$ for arbitrary fractional input arrival times
 with running time $\mathcal O(r(n) \log_2 n)$.
 We call $A'$ the \define{binary-search extension}
 of algorithm $A$.
 \begin{proof}
  We use the same notation as in the proof of \cref{n-times-int-general}.
  Denote the elements of $F$ by $\alpha_0, \dotsc, \alpha_{|F| - 1}$,
  where $\alpha_j < \alpha_{j + 1}$ for every $j \in \set{0, \dotsc, |F| - 2}$.
  Define the function
  \[d_{\text{int}} \colon F \to \N, \, \alpha \mapsto \delay(C_{\alpha}; a_{\alpha})\,.\]
 By \cref{obs-alpha-monotone}, the function $d_{\text{int}}$
 is monotonely decreasing in $\alpha$
 and assumes at most two values.

 By \cref{n-times-int-general}, there is $\alpha^* \in F$
 such that $C_{\alpha^*}$ is $S$-optimum for arrival times $a$.
 By \cref{bound-delay-alpha-a}, for all $\alpha \in F$, we have
 $\delay(C_{\alpha}; a) \leq \delay(C_{\alpha}; a_{\alpha}) + \alpha$,
 and by \cref{delay-alpha-eq}, equality holds for $\alpha = \alpha^*$.
 Hence, we have
 \[\alpha^* = \min \set{\alpha \in F \where
   d_{\text{int}}(\alpha) = d_{\text{int}}\Bkt{\alpha_{|F|-1}}}\,.\]
 Using binary search on $F$, we can determine $\alpha^*$
 in $\mathcal O(\log_2 |F|) = \mathcal O(\log_2 m)$ steps.
 \cref{table-binary} shows an example how to find $\alpha^*$.
 \end{proof}
\end{theorem}


==> settings/shortcref.tex <==
\makeatletter
% Macros adapted from this post: https://stackoverflow.com/a/964813/2747160
% Stores chip attribute:
%  #1: type of attribute (eg. name or technology)
%  #2: identificator of chip (ie. key in lookup table)
%  #3: attribute value
% Example: \registerShorthand{codename}{isztop}{Malygos}
% registers the "codename"-attribute of chip "isztop".
\newcommand\registerShorthand[2]{%
 \@namedef{shorthand-#1}{#2}%
}
% Access (previously) stored chip attribute:
%  #1: type of attribute (eg. name or technology)
%  #2: identificator of chip (ie. key in lookup table)
% Evaluates to the stored value if any or a default placeholder.
\newcommand\getShorthand[1]{%
  \@ifundefined{shorthand-#1}{%
   UNDEFINED%
  }{%
    \@nameuse{shorthand-#1}%
  }%
}

\registerShorthand{Definition}{Def.}
\registerShorthand{Section}{Sec.}
\registerShorthand{Theorem}{Thm.}
\registerShorthand{Proposition}{Prop.}
\registerShorthand{Lemma}{Lem.}
\registerShorthand{Corollary}{Cor.}
\registerShorthand{Remark}{Rem.}
\registerShorthand{Example}{Ex.}
\registerShorthand{Observation}{Obs.}
\registerShorthand{Claim}{Cl.}
\registerShorthand{Table}{Table}
\registerShorthand{Algorithm}{Alg.}
\registerShorthand{line}{l.}

\newcommand{\short}[1]{
 \@setnamecref{cref}{#1}{}{\expandafter\getShorthand}
}
\makeatother
\newcommand{\shortcref}[1]{\text{\short{#1}}\labelcref{#1}}

